A Newcomer In The PGAS World -- UPC++ vs UPC: A Comparative Study

A newcomer in the Partitioned Global Address Space (PGAS) 'world' has arrived in its version 1.0: Unified Parallel C++ (UPC++). UPC++ targets distributed data structures where communication is irregular or fine-grained. The key abstractions are global pointers, asynchronous programming via RPC, futures and promises. UPC++ API for moving non-contiguous data and handling memories with different optimal access methods resemble those used in modern C++. In this study we provide two kernels implemented in UPC++: a sparse-matrix vector multiplication (SpMV) as part of a Partial-Differential Equation solver, and an implementation of the Heat Equation on a 2D-domain. Code listings of these two kernels are available in the article in order to show the differences in programming style between UPC and UPC++. We provide a performance comparison between UPC and UPC++ using single-node, multi-node hardware and many-core hardware (Intel Xeon Phi Knight's Landing).

==> PGAS.tex <==
PGAS is a parallel programming model that has a logically partitioned global memory address space, where a portion of it is local to each process or thread. A special feature of PGAS is that the portions of the shared memory space may have an affinity for a particular process, thereby exploiting locality of reference \cite{UPCMPIOPENMPComparison2005,wikipediaDefPGAS}.

In the PGAS model, each node has access to both private and shared memory. Accessing the shared memory to either read or write data can imply inter-node communication  which is handled automatically by the runtime. Remote access to memory work in an  RDMA (Remote Direct Memory Access) fashion, using one-sided communication. However, most PGAS languages are built over a low-level communication layer which limits their physical capabilities. Thus, RDMA is available only if the underlying hardware and software support it.  

\iffalse
\begin{figure}[t]
\centering
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use
	\includegraphics[scale=0.32]{images/pgas.eps}
	% figure caption is below the figure
	\caption{PGAS Communication Model  \cite{PGAS_Definition} - Figure used with the courtesy of Marc Tajchman}
	\label{fig:PGAS_Communication_Model}       % Give a unique label
\end{figure}
\fi
In recent years several languages implementing the PGAS model have been proposed. UPC, which is essentially an extension of the C language, was one of the first ones and also one of the most stable \cite{PGAS_Definition}. Other members of the PGAS family of languages include the Fortran counterpart, Coarray Fortran \cite{coArrayFortran}, X10 \cite{x10}, and Cray Chapel \cite{crayChapel}. In addition, libraries such as Global Arrays \cite{globalArray} and SHMEM/OpenSHMEM \cite{openshmem} which implement PGAS functionality are available.

The key characteristics of UPC are: a parallel execution model of Single Program Multiple Data (SPMD); distributed data structures with a global addressing scheme, with static or dynamic allocation; operators on these structures, with affinity control; and copy operators between private, local shared, and distant shared memories.

Additionally, multiple open-source implementations of the UPC compiler and runtime environment are available, in particular Berkeley UPC \cite{BerkeleyUPC}, GCC/UPC \cite{GCCUPC} and CLANG/UPC\cite{clangUPC}.

==> nasBenchmark.tex <==
The NAS Benchmark \cite{NASOrigin} consists of a set of kernels that each provides a different way of testing the capabilities of a supercomputer. The NAS Benchmark was originally implemented in Fortran and C. We use both the Fortran and C implementations for OpenMP and MPI, as well as the UPC version of the benchmark \cite{UPCNAS}. For our study, we select four kernels: Integer Sort (IS), Conjugate Gradient (CG), Multi-Grid (MG), and Fourier Transformation (FT).

CG refers to the \textsl{conjugate gradient} method used to compute an approximation to the smallest eigenvalue of a large, sparse, symmetric positive definite matrix. %This kernel is typical for unstructured grid computations in that it tests irregular all-to-all communication arising in sparse matrix-vector multiplication.

MG is a simplified \textsl{multigrid} kernel. Multigrid (MG) methods in numerical analysis solve differential equations using a hierarchy of discretizations. %For example, a class of techniques called multiresolution methods, are very useful in (but not limited to) problems exhibiting multiple scales of behavior. MG tests both short-and all-to-all data exchange as well as local memory accesses.

FT is a three-dimensional partial differential equation solver using \textsl{Fast Fourier Transformations}. This kernel performs the essence of many spectral codes. It is a rigorous test of all-to-all communication performance. %\cite{NASOrigin}

IS represents a large \textsl{integer sort}. This kernel performs a sorting operation that is important in {particle method codes. It evaluates both integer computation speed and communication performance. %\cite{NASOrigin}

CG, IS, MG and FT  are selected  because they are the most relevant ones: stressing memory, communication and computation. They involve very different communication patterns, which is important for evaluating the performance of the selected languages (see Section \ref{results}). The other kernels in the NAS Benchmark are of limited relevance to this study. See \cite{NASOrigin} for their descriptions. 



==> previous.tex <==



